Multi-way Graph Signal Processing on Tensors: Integrative analysis of irregular geometries

Graph signal processing (GSP) is an important methodology for studying data residing on irregular structures. As acquired data is increasingly taking the form of multi-way tensors, new signal processing tools are needed to maximally utilize the multi-way structure within the data. In this paper, we review modern signal processing frameworks generalizing GSP to multi-way data, starting from graph signals coupled to familiar regular axes such as time in sensor networks, and then extending to general graphs across all tensor modes. This widely applicable paradigm motivates reformulating and improving upon classical problems and approaches to creatively address the challenges in tensor-based data. We synthesize common themes arising from current efforts to combine GSP with tensor analysis and highlight future directions in extending GSP to the multi-way paradigm.

==> gsp_tensors.tex <==
Classical $D$-dimensional Fourier analysis provides a template for constructing unified geometries from various data sources. The $D$-dimensional Fourier transform applies a 1-dimensional Fourier transform to each axis of the data sequentially. For example, a 2D DFT applied to an $n_1 \times n_2$ image $\M{X}$ is %(represented as the matrix $\mathbf{X}$ with $\mathbf{X}_{i,j} \in [0,255]$) is 
\begin{equation}
\label{eq:dft2d}
    \text{2D-DFT}\{\M{X}\}=\mathrm{DFT}_c(\mathrm{DFT}_r(\mathbf{X})) = \mathrm{DFT}_r(\mathrm{DFT}_c(\mathbf{X}))=\M{U}_{n_1}\M{X}\M{U}_{n_2}\Tra,
\end{equation} 
where $\mathrm{DFT}_{n_1}$ ($\mathrm{DFT}_{n_2}$) applies the DFT to the rows (columns) of $\mathbf{X}$ %$\mathrm{DFT}_{n_2}$ applies the DFT to the columns of $\mathbf{X}$. 
and $\M{U}_{n}$ denotes an $n$-point DFT matrix. %The symbol $\cong$ denotes an  \emph{isomorphism} between the left and right hand sides of~\Cref{eq:dft2d}; the order that each 1-dimensional DFT is taken is inconsequential, as the resulting coefficients are the same up to a permutation. 
This 2D transform decomposes the input into a set of plane waves.

% to Jay: permutation comment and isomorphism is only relevant if this was in vec form but it is not, so I removed it.
%begin{equation}
%\label{eq:dft2d}
%    \text{2D-DFT}\{\M{X}\}=\mathrm{DFT}_c(\mathrm{DFT}_r(\mathbf{X})) \cong \mathrm{DFT}_r(\mathrm{DFT}_c(\mathbf{X}))=\M{U}_{n_1}\M{X}\M{U}_{n_2}\Tra,
%\end{equation} 
%where $\mathrm{DFT}_{n_1}$ ($\mathrm{DFT}_{n_2}$) applies the DFT to the rows (columns) of $\mathbf{X}$ %$\mathrm{DFT}_{n_2}$ applies the DFT to the columns of $\mathbf{X}$. 
%and $\M{U}_{n}$ denotes an $n$-point DFT matrix. The symbol $\cong$ denotes an  \emph{isomorphism} between the left and right hand sides of~\Cref{eq:dft2d}; the order that each 1-dimensional DFT is taken is inconsequential, as the resulting coefficients are the same up to a permutation. This 2D transform decomposes the input into a set of plane waves.


The 2D-GFT is algebraically analogous to the 2D-DFT. For two graphs $\G^{(1)}$ and $\G^{(2)}$ on $n_1$ and $n_2$ vertices, a 2D graph Fourier transform of $\M{X}\in \Real^{n_1\times n_2}$ is
\begin{equation}
\label{eq:2dgft}
\text{2D-GFT}(\M{X}) =\mathrm{GFT}_{n_1}(\mathrm{GFT}_{n_2}(\M{X})))=\mathrm{GFT}_{n_2}(\mathrm{GFT}_{n_1}(\M{X})).
\end{equation}
\cite{Sandryhaila2014} suggested the 2D-GFT as a method for efficiently processing big-data. We will elaborate its similarity to the DFT shortly but 
%Its similarity to the DFT will be mathematically elaborated subsequently,
 to provide brief intuition we note that when $\G^{(1)}=\mathcal{P}^{n_1}$ and $\G^{(2)}= \mathcal{P}^{n_2}$, i.e., they are \emph{path graphs} on $n_1$ and $n_2$ vertices, this transform is equivalent to a 2D DFT~\cite{Sandryhaila2014}. 

In the following, we describe Multi-way Graph Signal Processing (MWGSP), a framework for $D$-dimensional signal processing on coupled and irregular domains, which  enables holistic data analysis by considering relational structures on potentially {\em all} modes of a mutli-way signal. MWGSP encompasses traditional graph signal processing while extending fundamental GSP tools such as graph filters to $D$-dimensions. Furthermore, because graphs can be used to model discrete structures from classical signal processing, MWGSP forms an intuitive superset of discrete signal processing on domains such as images or video. 

\subsection{Tensors}
%\emph{Tensors} are the primary tool for representing $D$-dimensional signals. 
\emph{Tensors} are both a data structure representing $D$-dimensional signals, 
%that generalizes matrices to $D$-dimensions
as well as a mathematical tool for analyzing multilinear spaces. We use both perspectives to formulate MWGSP.
In this paper, we adopt the tensor terminology and notation used by \cite{KoldaBader2009}.
\subsubsection{Tensors as a $D$-dimensional array}
We call the number of ways or modes of a tensor its {\em order}. Vectors are tensors of order one and denoted by boldface lowercase letters, e.g.\@ $\V{a}$. Matrices are tensors of order two and denoted by boldface capital letters, e.g.\@ $\M{A}$. Tensors of higher-order, namely order three and greater, we denote by boldface Euler script letters, e.g.\@ $\T{A}$. If $\T{A}$ represents a $D$-way data array of size $n_1 \times n_2 \times \cdots \times n_D$, we say $\T{A}$ is a tensor of order $D$.

There are multiple operations to reshape tensors. \emph{Vectorization} maps the elements of a matrix into a vector in column-major order. That is, for $\M{X}\in \Real^{n_1\times n_2}$, $$\vec(\M{X}) = [ \M{X}_{1,1}, \ldots,  \M{X}_{n_1,1}, \M{X}_{1,2}, \ldots, \M{X}_{n_1,2}, \ldots,  \M{X}_{1,n_2}, \ldots,  \M{X}_{n_1,n_2}]^\mathrm{T}.$$ A tensor mode-$d$ vectorization operator, $\vec_d(\T{X})$ is similarly defined by stacking the elements of $\T{X}$ in mode-$d$ major order. 
Let $\mathrm{ten}(\V{x},\ell,\{n_1,\ldots,n_D\}) = \T{X}$ be the $\ell$-th \emph{tensorization} of $\V{x}$, which is the inverse of the $\ell$-major vectorization of $\T{X}$.
Denote by $n\setminus \ell = \prod_{i=1}^{\ell-1} n_i \prod_{j=\ell+1}^D n_j$ the product of all factor sizes except for the $\ell$-th factor. 
 Then, let $\mathrm{mat}(\T{X},\ell) = \M{X}^{(\ell)} \in \Real^{n_\ell \times N\setminus \ell}$ be the mode-$\ell$ matricization of $\T{X}$ formed by setting the $\ell$-th mode of $\T{X}$ to the rows of $\M{X}^{(\ell)}$, vectorizing the remaining modes to form the columns of $\M{X}^{(\ell)}$ as in Fig.~\ref{fig:tensor}(f). %\TODO{Remove redundant notation introduction in later text}


\begin{mdframed}[userdefinedwidth=\linewidth,align=center,usetwoside=false,rightmargin=-0.2in,
linecolor=blue,linewidth=1pt,frametitle = {Order-3 tensors}]
\small
%The $N$-dimensional $N$-tensor $\T{X}$ (also known as an $N$th order tensor) is composed of $N$ modes.  
For simplicity, we briefly review some tensor terminology for the $3$-way tensor $\T{X}\in \mathbb{C}^{n_1 \times n_2\times n_3}$. 
The size of each mode is denoted by $n_i$, with $n_1$ being the number of columns, $n_2$ the number of rows, and $n_3$ being the number of \emph{tubes}~\cite{KoldaBader2009}. Video and time-series recording of matrix valued signals are a common application for tensors of this form (\cref{fig:tensor}(a)). In videos, the first and second modes of the tensor encode pixel values for each frame, while the third axis indexes the frames in time. 
We can \emph{slice} a video tensor to produce different views of the data. A \emph{frontal slice} is the matrix $\T{X}_{:,:,k}$, formed by selecting the $k$-th frame of the video as in \cref{fig:tensor}(b).
Though each frame matrix is intuitively an image, we can also create matrices using \emph{horizontal slices}, $\T{X}_{i,:,:}$, which for a video produces a matrix (viewable as an image) that shows the time evolution of the $i$-th row of pixels in the input as in \cref{fig:tensor}(c); similarly, the \emph{lateral slice} $\T{X}_{:,j,:}$ contains the time evolution of one column of pixels of the input as in \cref{fig:tensor}(b). 
Finally, one can consider 2D and 3D indexing of 3rd order tensors, with, for example, the \emph{fiber} $\T{X}_{i,j,:}$ returning a $n_3$ dimensional time-series vector of the value of the $i,j$th pixel of each frame shown in \cref{fig:tensor}(e), while $\T{X}_{i,j,k}$ is a single number corresponding to the value of pixel $i,j$ in frame $k$.  

\begin{comment}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/tensor.pdf}
    \caption{From left to right: Tensor of order 3 - $\mathcal{T}$, fibers along third mode -  $\mathcal{T}_{ij\cdot}$, slices of first mode -  $\mathcal{T}_{i\cdot\cdot}$, slices of second mode - $\mathcal{T}_{\cdot j \cdot}$. }
    \label{fig:tensor}
    \vspace{-0.2cm}
\end{figure}
\end{comment}
    \centering
    \includegraphics[width=0.95\linewidth]{figures/tensor2.pdf}
    \captionof{figure}{\small (a) Tensor, (b) frontal (c) lateral and (d) horizontal slices. (e) Two tubalar fibers corresponding to pixels in (a). (f) Mode-1 matricization concatenates all frontal slices side by side (g) CP decomposition.}
    \label{fig:tensor}
    \vspace{-0.2cm}

\end{mdframed}


%. In this setting, learned or assigned graphs provide relational abstractions for the rows, columns, and higher order modes of data matrices and tensors. The data may be modeled by a product graph where each element of the dataset is a vertex, or the modal graphs can be treated separately. This general framework includes signal and image processing, and GSP as special cases.


%However, in this survey, we are more focused on algorithms that consider the unification of many irregular geometries, absent a predefined temporal or regular axis. These algorithms are by definition more versatile- as we previously discussed, an algorithm designed for GFTs can be directly applied to classical discrete analysis by considering particular graphs, though they may underperform in temporal settings due to lackof specialization.


\subsubsection{Tensor products}
Up to this point we have avoided explicitly constructing  $D$-dimensional transforms.
In the 2D case, applying a two-dimensional transform is calculated via linear operators as in~(\ref{eq:dft2d});  generalizing to higher-order tensors requires multilinear operators.   
Therefore, we introduce the \emph{tensor product} and its discrete form, the \emph{Kronecker product}. These products are powerful tools for succinctly describing $D$-dimensional transforms.

The great utility of the tensor product is that it simultaneously transforms spaces alongside their linear operators. This is the so-called \emph{universal property} of the tensor product.  In brief, it states that the tensor product of two vector spaces $V$ and $W$ is the unique result  of a bilinear map $\varphi : V \times W \rightarrow V \otimes W$.  The power in $\varphi$ is that it uniquely factors any bilinear map on $V\times W$ into a linear map on $V \otimes W$. The universal property implies that the tensor product is symmetric: $V \otimes W$ is a canonical isomorphism of $W \otimes V$.  Though the tensor product is defined in terms of two vector spaces, it can be applied repeatedly to combine many domains, so we generically refer to it as a product of many spaces.

In this paper, we are particularly concerned with the tensor product on Hilbert spaces $\mathcal{H}^{(k)}, k=1,\ldots, D$. These metric spaces include both continuous and discrete Euclidean domains from classical signal processing, as well as the non-Euclidean vertex domain. Since tensor products on Hilbert spaces produce Hilbert spaces, we can combine time, space, vertex, or other signal processing domains via the tensor product and remain in a Hilbert space. Under some constraints, an orthonormal basis for the product of $D$ Hilbert spaces is admitted directly by the tensor product of the factor spaces.

To obtain a $D$-dimensional GFT, we note that \begin{enumerate*} \item these discrete 1D transforms are linear, and \item the domain of a $D$-dimensional GFT is the tensor product of $D$ Hilbert spaces. \end{enumerate*} Thus, by the universal property of tensor products, a multidimensional GFT can be obtained by a multilinear transformation of the 1D transforms. Remarkably, the new transform may be computed \emph{without computing a product space.} However, as the GFT amounts to a change of basis, its multidimensional extensions immediately yield a basis that encodes the geometry of the product space.
\paragraph*{Kronecker products}
The Kronecker product produces the matrix of a tensor product with respect to a standard basis and 
generalizes the outer product of vectors $\V{x}\V{y}^*$ for $\V{x}\in\Complex^{m}$ and $\V{y} \in \Complex^{n}$. For analogy, it is common to use the same notation to denote the Kronecker and tensor product.
%, and the Kronecker product of two matrices $\M{A}^{(1)} \in \Complex^{n_1\times m_1}$ and $\M{A}^{(2)} \in \Complex{}^{n_2\times m_2}$ is the $n_1n_2\times m_1m_2$ matrix 
%$${\displaystyle \Mn{A}{1}\otimes \Mn{A}{2}  ={\begin{bmatrix}\MnE{A}{1}{11}\Mn{A}{2} &\cdots &\MnE{A}{1}{1m_1}\Mn{A}{2}\\\vdots &\ddots &\vdots \\\MnE{A}{1}{n_11}\Mn{A}{2} & \cdots&\MnE{A}{1}{n_1m_1}\Mn{A}{2} \end{bmatrix}}.}$$
The Kronecker product is associative. Consequently for a  sequence of $D$ matrices $\M{M}^{(k)} \in \Complex^{n_k \times n_k}$ for $k=1,\ldots,D$
%\begin{equation}
%\begin{split}
%\M{A}^{\otimes} = \bigotimes_{k=1}^d \M{A}^{(k)} &=  \M{A}^{(1)}\bigotimes_{k=2}^d \M{A}^{(k)} = \left(\bigotimes_{k=1}^{d-1} \M{A}^{(k)}\right)\Kron \M{A}^{(d)}\\ &= \M{A}^{(1)}\Kron \ldots \Kron \M{A}^{(d)}.
%\label{eq:general_kronecker_product}
%\end{split}
%\end{equation}
\begin{equation}
\begin{split}
\M{M} = \bigotimes_{k=1}^D \M{M}^{(k)} =  \M{M}^{(1)}\bigotimes_{k=2}^D \M{M}^{(k)} = \left(\bigotimes_{k=1}^{D-1} \M{M}^{(k)}\right)\Kron \M{M}^{(D)} = \M{M}^{(1)}\Kron \cdots \Kron \M{M}^{(D)}.
\label{eq:general_kronecker_product}
\end{split}
\end{equation}
It is important to note that the Kronecker product is in general non-commutative.

The Kronecker product has many convenient algebraic properties for computing multidimensional transforms.
Vectorization allows one to define matrix multiplication as a linear transformation% using the ``vec trick,'' 
\begin{equation}
    \vec(\M{C}\M{X}\M{B})=(\M{B}\Tra\Kron\M{C})\vec{(\M{X})},
    \label{eq:vectrick}
\end{equation}
assuming that the dimensions of $\M{C},\M{X},\M{B}$ are compatible so that $\M{C}\M{X}\M{B}$ is a valid operation.

This identity is a discrete realization of the universal property of tensors, and shows that the Kronecker product corresponds to a bilinear operator. We will use this  identity to \begin{enumerate*} \item construct multi-dimensional discrete Fourier bases, and \item  decompose multiway algorithms for computational efficiency. \end{enumerate*}

\subsubsection{Constructing multiway Fourier bases}
\TODO{Jay is it necessary to do this for 2D-DFT? Why not so directly for 2D-GFT?}
A 2D-DFT basis for an $n_1\times n_2$ grid is immediate from~(\ref{eq:dft2d}),(\ref{eq:vectrick}), as 
$$\vec(\text{2D-DFT}(\M{X})) = \vec(\M{U}_{n_1}\M{X}\M{U}_{n_2}\Tra)= (\M{U}_{n_1}\Kron\M{U}_{n_2})\vec(\M{X}).$$ 
We also use (\ref{eq:vectrick}) to show the permutation equivalence of multidimensional Fourier transforms, as for any Kronecker product of two matrices $\M{B}$ and $\M{C}$ there always exists a pair of permutation matrices $\M{P}_1$ and $\M{P}_2$ such that $\M{P}_1(\M{B}\Kron\M{C})\M{P}_2=(\M{C}\Kron\M{B})$~\cite{horn1994topics}.
 Thus, $\M{U}_{n_2}\Kron\M{U}_{n_1}$ and $\M{U}_{n_1}\Kron\M{U}_{n_2}$ are 2D-DFT bases for the row-major and column-major vectorization of a signal.

%The symbol $\cong$ denotes an  \emph{isomorphism} between the left and right hand sides of~\Cref{eq:dft2d}; the order that each 1-dimensional DFT is taken is inconsequential, as the resulting coefficients are the same up to a permutation.

 These observations for the DFT apply directly to construct a 2D GFT.
 If $\M{\M{\Psi}}^{(1)}$ and $\M{\M{\Psi}}^{(2)}$ are Fourier bases for graph signals on any two graphs $\G_1$ and $\G_2$, a 2D GFT basis is $\M{\M{\Psi}}^{(1)} \Kron \M{\M{\Psi}}^{(2)}$. This is a single orthonormal basis of dimension $|\Vc^{(1)}||\Vc^{(2)}|\times |\Vc^{(1)}||\Vc^{(2)}|$, which can be used to describe a 2D graph signal $\M{X}\in\Real^{n_1\times n_2}$ in the geometry of a single graph by the \TODO{GFT} $(\M{\M{\Psi}}^{(1)}\Kron\M{\M{\Psi}}^{(2)})\vec(\M{X}) = \hat{\V{x}}$. Yet, unlike the DFT, where it is clear that increasing dimension yields grids, cubes, and hypercubes, interpreting the geometry of $\M{\M{\Psi}}^{(1)} \Kron \M{\M{\Psi}}^{(2)}$ is less intuitive. For this, we must turn to a \emph{graph product}.




\paragraph*{Product graphs} MWGSP relies on a graph underlying each mode of the given tensor data. The question is: What joint geometry arises from these graphs, and what multilinear operators exist on this joint graph structure? Our approach is to construct a multidimensional graph $\G$ over the entirety of a data $\T{X}$ as the \emph{product graph} of a set of \emph{factor} graphs $G = \{\G^{(1)},\ldots, \G^{(D)}\}$. 

For example, if $\T{X}$ contains the results of a $n_3$ sample longitudinal survey of $n_2$ genes on a cohort of $n_1$ patients, then the intramodal relationships of $\T{X}\in\Real^{n_1\times n_2\times n_3}$ are modeled by separate graphs $\G^{(1)}$, in which each patient is a vertex, $\G^{(2)}$, in which each gene is a vertex, and $\G^{(3)}$, which represents time as a path graph on $n_3$ vertices. We will use this example throughout this section, though our derivation generalizes to any order tensor.

While one could treat matrix-valued slices of $\T{X}$ as signals on each individual graph or perform a multilinear GFT over the data, we use the graph product to model $\T{X}$ as a single graph signal. We begin by constructing the vertices of $\G$, which for all graph products is performed by assigning a single vertex to every element in the Cartesian product of the factor vertex sets  i.e., $\Vc = \Vc^{(1)} \Cart \ldots \Cart \Vc^{(D)}$. Thus, the vertex set of $\G$ is of cardinality $n=\prod_{k=1}^D n_k$. For example, our longitudinal survey will be modeled by the product graph $\G$ on $n = n_1n_2n_3$ vertices. As a Cartesian product, the elements of $\Vc$ can be expressed as (\emph{patient}, \emph{gene}, \emph{time}). The experimental observation tensor can be modeled as a graph signal $\vec(\T{X})$ in $\Real^{n}$, $\V{x}=\vec({\T{X}})$.\footnote{We can do this because the vectorization $\vec({\T{X}})$ is isomorphic to $\T{X}$, which can be shown using \cref{eq:vectrick}.} 

Our next step is to learn the geometry of $\G$. This geometry is given by a multilinear mapping of the edge sets (weights) of the factor graphs into a single set of product edges (weights). There are a variety of graph products, each of which differs from each other only in the construction of this map. We focus on the \emph{Cartesian graph product} as it is the most widely employed in multi-way algorithms. However, we note that that other products such as the tensor and strong graph products each induce novel edge topologies that warrant further exploration for multiway graph signal processing \citep{imrich2000product}. 



 
% \footnote{Here $\circ$ is a generic product operation on graphs.}
% \begin{align*}
% \G^\circ = \G^{(1)}\circ\cdots\circ\G^{(D)}
% \end{align*} is the set of all unique $D$-tuples, \begin{align*}
% V(\G) = V(\G^{(1)}) \Cart \cdots \Cart V(\G^{(D)}) = \left\{(v^{(1)},\ldots,v^{(D)}) : \begin{array}{l}
%     v^{(\ell)} \in V(\G^{(\ell)})\\
%     \forall ~\ell\in\{1,\ldots,D\} 
%   \end{array}\right\}.
% \end{align*} 
%\begin{align*}
%\G^\circ = \G^{(1)}\circ\cdots\circ\G^{(D)}
%\end{align*} is the set of all unique $D$-tuples, \begin{align*}
%V(\G) &= V(\G^{(1)}) \Cart \cdots \Cart V(\G^{(D)})\\ & = \left\{(v^{(1)},\ldots,v^{(D)}) : \begin{array}{l}
%    v^{(\ell)} \in V(\G^{(\ell)})\\
%    \forall ~\ell\in\{1,\ldots,D\} 
%  \end{array}\right\}.
%\end{align*} 
%\Jay{Gal}{Does this make more sense?}


%%%%%%%%%%%%%%%%%%% 
\paragraph*{Cartesian graph products}
%%%%%%%%%%%%%%%%%%% 
We denote the Cartesian product of $D$ graphs as
\begin{align}
\G = \GCart\limits_{\ell=1}^D \G^{(\ell)} = \G^{(1)}\Gcart\cdots\Gcart\G^{(D)}.
\end{align}
The Cartesian graph product is intuitively an XOR product since for any two vertices 
\begin{align}\left\{v=\left(v^{(1)},\ldots,v^{(D)}\right),u=\left(u^{(1)},\ldots,u^{(D)}\right)\right\}\subset \Vc,
\end{align}
the edge $(v,u)$ 
exists if and only if there exists a single $i$ such that $(v_i,u_i) \in \Ec^{(i)}$ and $v_\ell = u_\ell$ for all $\ell\neq i$. In other words, the vertices of $\G$ are connected if and only if exclusively one pair of factor vertices are adjacent and the remaining factor vertices are the same.~\Cref{fig:product_graphs}a illustrates the generation of an $n_1\times n_2$ 2D grid graph via the product of two path graphs on $n_1$ and $n_2$ vertices. 

The XOR product can induce topological properties such as regularity onto a graph. Since the path graph basis is well-characterized as a discrete Fourier basis, it is a convenient tool for including Euclidean domains in multi-way analysis.  For example, we can model time series and longitudinal graph signals as a single vector using a path graph product. In the case of our gene expression data $\T{X}$, the product of the gene and patient mode graphs with a path on $n_3$ vertices, i.e., $\G^{(1)}\Gcart\G^{(2)}\Gcart \mathcal{P}^{n_3}$, models the data by treating the temporal mode as a sequence. One can intuit this operation as copying $\G^{(1)}\Gcart\G^{(2)}$ $n_3$ times and connecting neighborhoods between each copy.

\paragraph*{Product graph matrices}
The Kronecker product links graph shift operators on Cartesian product graphs to the corresponding operators on the factors. For this purpose, we introduce the \emph{Kronecker sum} of $D$ matrices $\M{A}^{(k)} \in \Complex^{n_k\times n_k}$ for $k=1,\ldots,D$ is 
 \begin{equation}
 \M{A}= \bigoplus_{k=1}^D \M{A}^{(k)} = \sum_{k=1}^{D} \M{I}_{n_{>k}}\Kron{}\M{A}^{(k)}\Kron{}\M{I}_{n_{<k}},\label{eq:general_kronecker_sum} \text{where} ~ n_{>k} = \prod_{\ell=k+1}^D n_\ell, ~ \text{and}~ n_{<k} = \prod_{\ell=1}^{k-1} n_\ell\nonumber.
 \end{equation}
 The joint adjacency matrix $\M{A}$ and graph Laplacian $\M{\mathcal{L}}$ are constructed by the Kronecker sum of their corresponding factor graph matrices.% are computed by the Kronecker sum of the factors.
~The eigensystem of a Kronecker sum is generated by the pairwise sum of the eigenvalues of the factors and the tensor product of the factor eigenbases  \citep[][Thm. 4.4.5]{horn1994topics}. Thus, the Fourier basis for $\G$ is immediate from the factors.
For $k=1,\ldots,D$~let $(\lambda_{\ell_k},\M{\Psi}_{\ell_k})$ be the $\ell_k$th eigenpair of $\M{\mathcal{L}}^{(k)}$ for $0\leq\ell_k\leq n_k-1$
Then let $I_{\ell} = (\ell_1,\ldots,\ell_D) \in [n_1]\times\ldots \times [n_D]$
%To formalize this, it is easiest to multi-index the eigensystem,  
be a multi-index to the $\ell$th eigenpair of $\M{\mathcal{L}}$.  The product graph Fourier basis is then
\begin{align}
\label{eq:general_kron_sum_eigensystem}
\left(\lambda_{I_{\ell}},\M{\Psi}^{}_{I_{\ell}}\right) = \left(\sum_{k=1}^D \lambda^{(k)}_{\ell_k}, \bigotimes_{k=1}^D \M{\Psi}^{(k)}_{\ell_k}\right).
\end{align} 
This spectral characterization of the Cartesian product graph implies that all graphs which admit a Cartesian factorization over the same set of graphs are isomorphic.  Thus, like the D-dimensional DFT, D-dimensional GFTs are equivalent up to a permutation of the input signal.

%\paragraph{\TODO{additional notations we may need}} Let $\T{A}$ be a tensor in $\Real^{n_1 \times n_2 \times \cdots \times n_D}$ and $\M{B}$ be a matrix in $\Real^{m \times n_d}$. The {\em d-mode (matrix) product} of the tensor $\T{A}$ with the  matrix $\M{B}$, is the tensor denoted by $\T{A} \times_{d} \M{B} \in \mathbb{R}^{n_1 \times \cdots \times n_{d-1} \times m \times n_{d+1} \times \cdots \times n_D}$ whose $(i_1, i_2, \cdots, i_{d-1}, j, i_{d+1}, \cdots, i_D)$th element is given by 
%\begin{eqnarray}
%(\T{A} \times_d \M{B})_{i_1\ldots i_{d-1} j i_{d+1} \cdots i_D} & = & \sum_{i_d = 1}^{n_d} \ME{a}{i_1i_2\cdots i_D}\ME{b}{j i_d}, \quad \textrm{for } j \in \{1, \ldots, m\}
%\end{eqnarray}
%The vectorization of the $d$-mode product $\T{A} \times_{d} \M{B}$ can be expressed as
%\begin{equation}
%\begin{split}
%\label{eq:vec_identity}
%\vec (\T{A} &\times_d \M{B}) 
% =  (\M{I}_{n_D} \Kron \cdots \Kron \M{I}_{n_{d+1}}\Kron \M{B} \Kron \M{I}_{n_{d-1}} \Kron \cdots \Kron \M{I}_{n_1} )\V{a},
%\end{split}
%\end{equation}
%where $\M{I}_p$ is the $p$-by-$p$ identity matrix and $\Kron$ denotes the Kronecker product between two matrices. %The identity given in \Eqn{vec_identity} generalizes the well known formula for the column-major vectorization of a product of two matrices, namely $\vec(\M{B}\M{A}) = (\M{I}\Kron\M{B})\V{a}$.

% \TODO{It would be good to summarize here by introducing a multi-way GFT transform on tensors, generalizing ~(\ref{eq:3dgft}) from 3D, and refering to its joint graph laplacian and eignedecomposition from the equations above. As ihn, now that we have introduced all of this math, we can finally define this very important all encompassing transform.}
\paragraph{Efficient multiway GSP by graph factorization}

Multi-way product graphs are often much larger than their factors, as the cardinality of the product vertex set is the product of the number of vertices in each factor. On the surface, this appears to inflate the computational challenge of multiway graph signal processing.  However, the product graph structure actually yields efficient algorithms.  With small adjustments to fundamental operations like matrix multiplication, in the best case one can effectively reduce the computational burden of an order $D$ tensor with $n = \prod_{\ell=1}^Dn_\ell$ total elements to a sequence of problems on $n^{(1/D)}$ elements. The computational strategy is to apply~\Cref{eq:vectrick} and its order-$D$ generalization to avoid storing and computing large product graph operators. 

We introduce the order-$D$ form of~\Cref{eq:vectrick} via an algorithm. Given a sequence of operators $\M{M}^{(\ell)}\in \Real^{n_\ell},~\ell=1,\ldots, D$, an efficient algorithm for computing \begin{align}\V{y}= \bigotimes_{k=1}^D \M{M}^{(\ell)}\vec(\T{X})\label{eq:directapplication}\end{align} proceeds by applying each $\M{M}^{(\ell)}$ to the corresponding mode-wise matricization of $\T{X}$. An informal version of this algorithm is provided in~\Cref{alg:mode-D}.
\begin{algorithm}
\caption{$D$-tensor compression}
\begin{algorithmic}[1]
\State Initialize $\T{Y} =\T{X}$

\For{$\ell=1,\ldots,D$}
\State  Matricize: $\M{Y}^{(\ell)} = \mathrm{mat}(\T{Y},\ell)$
\State Factor update: $\M{Y}^{(\ell)} = \M{M}^{(\ell)\Tra} \M{Y}^{(\ell)}$
\State  Reform tensor: $\T{Y} = \mathrm{ten}(\M{Y}^{(\ell)},\ell,\{n_1,\ldots,n_D\})$
\EndFor
\State Vectorization: $\V{y} = \mathrm{vec}(\T{Y}).$
\end{algorithmic}
\label{alg:mode-D}
\end{algorithm}
As a sequential product of an $n_\ell\times n_\ell$ matrix with an $n_\ell \times n \setminus \ell$ matrix, this method can dramatically improve the cost of algorithms that depends on matrix multiplication. Further, the number of operations are only dependent on computations over smaller factor matrices, which allows one to perform costly computations for smaller factors as a compression of the larger product. As an example, consider the computational burden of computing and applying a graph Fourier basis for a product graph $\G$ on $n=\prod_{\ell=1}^D n_\ell$ nodes. In the worst case, ~\Cref{alg:mode-D} is as fast as directly computing~\Cref{eq:directapplication}. However, in the near-optimal case where $n_\ell=n_k$ for all $k=1,\ldots,D$, one computes $D$ graph Fourier bases of size $\sqrt[D]{N} \times \sqrt[D]{N} $.  Thus, obtaining a compression of the eigenbasis for a product graph shift operator asymptotically requires $\mathbf{O}(\sqrt[D]{N}^3)$ operations. Indeed, when $D=3$ and $n_1=n_2=n_3=\sqrt[3]{N},$ we obtain an asymptotically linear compression of a graph Fourier basis for $\G$. \TODO{Apply a GFT}

\paragraph*{Edge density}
We briefly comment on how the graph edge density impacts the scalability of signal processing algorithms for multiway data. Matrix equations can be efficiently solved by iteratively computing a sparse matrix-vector products. The computational complexity of such algorithms, which include fundamental techniques such as Krylov subspace methods and polynomial approximation, typically depend linearly on the number of edges in the graphs, e.g.,\@ \cite{Hammond2011,Shahid2016, Chi2017a, grassi2017time,Tremblay2016}. This dependency suggests using the sparsest possible graph that still captures the main similarity structure along each mode. Indeed, a common strategy is to construct sparse Laplacian matrices \cite{Shahid2016} or edge-incidence matrices \cite{Chi2017a}, using $k$-nearest-neighbor graphs which produce edge sets whose cardinality is linear in the number of nodes. Additional strategies for sparse graph construction have also been proposed \cite{mateos2019connecting}. Yet, given sparse factors graph, there is no guarantee that the product will be sparse. Thus, major efficiency gains for multiway algorithms can be made by replacing iterative matrix-vector multiplications (both sparse and dense) with a sequence of factor graph sparse matrix-vector multiplications using the algorithm introduced in \TODO{backref}.




\begin{mdframed}[userdefinedwidth=\linewidth,align=center,usetwoside=false,rightmargin=-0.2in,
linecolor=blue,linewidth=1pt,frametitle = {Multi-way Filters}]
\label{sec:multi-way_filters}
%\linespread{1.5}
\small{
It is natural to define spectral filters for multiway graph signals on the product $\G^\square$ as a function over the product graph eigenvalues $g: \Lambda^\square \mapsto \Real{}$ as if they are traditional spectrally defined GSP filters. For example, the filter in ~\cref{fig:product_graphs}b illustrates the effect of the product adjacency matrix on a delta signal. Since these functions operate on the product eigenvalues, they directly consider the edge topology induced by a particular choice of product. 
Yet, it is feasible to develop filters for multiway graph signals on $\G^\square$ that are defined by multivariate functions $g^\prime : \Lambda^{(1)}\Cart\cdots\Cart\Lambda^d \mapsto \Real{}$. These multivariate filters are split into two classes: separable and nonseparable.

 Separable filters have multivariate response functions that can be written as the product of separate univariate functions. In the $D=2$ case, a separable filter for the product graph could be written as $\left(\M{T}^{(1)}\Kron{}\M{T}^{(2)}\right)\V{x}$ in which $\M{T}^{(1)} = \M{\M{\Psi}}^{(1)} t^{(1)}(\M{\Lambda}^{(1)}) \M{\M{\Psi}}^{(1)*}$ and $\M{T}^{(2)} = \M{\M{\Psi}}^{(2)} t^{(2)}\left(\M{\Lambda}^{(2)}\right) \M{\M{\Psi}}^{(2)*}.$ Since this operator is bilinear, we can treat its operation as an order-independent\footnote{this does not imply the Kronecker product is commutative but rather that it corresponds to a commutative linear operator} unimodal filtering of $\V{x}$~(\ref{eq:vectrick}). If $\M{T}^{(1)}$ and $\M{T}^{(2)}$ are both filters defined in \TODO{a} Laplacian eigenbasis of their respective graph, then the tensor product $\left(\M{T}^{(1)}\Kron{}\M{T}^{(2)}\right)$ is also diagonalized by the product eigenbasis. \TODO{Thus, this filter is merely a reweighting of the product graph eigenbasis.} Importantly, however, it adds a degree of freedom that cannot be obtained using the 1D eigenvalues of $\Lambda^\square$. 
 In~\Cref{fig:product_graphs}e, we demonstrate the application of a product of mode-wise heat filters to a graph signal on a grid~(\cref{fig:product_graphs}d top) and to a time-vertex signal which is a dynamic mesh~(\cref{fig:product_graphs}d bottom). While there is a choice of $\tau_1$ and $\tau_2$ such that certain regions of this filter can be computed from a heat kernel on the Cartesian product graph spectrum, such an approach abandons the flexibility of bilinear filtering. 
 By separability, each mode can be analyzed independently of the other by setting the appropriate $\tau_k$ to 0. This enables analyzing a joint signal along each mode independently, for example by filtering out high frequency structure along one domain while preserving the frequency content of the other mode.
 
 Nonseparable filters cannot be designed from separate univariate filters on each mode. This class of filters encompasses a broad class of functions that include many filters defined in terms of the product graph eigenvalues, as well as multivariate functions (\cref{fig:product_graphs}f). Indeed,~\cite{grassi2017time} find that one cannot in general describe PDEs that describe diffusion, wave, or disease propagation with separable filters, as the relation between frequencies is not independent. %In the rightmost column of~\cref{fig:product_graphs}c, a nonseparable wave filter is applied to a graph signal.
 }
 \end{mdframed}
 
 \begin{figure*}
     \centering
    \includegraphics[width=0.9\linewidth]{figures/horz_graph_filters_ver2.png}
    \captionof{figure}{\small Multi-way graphs, signals and spectral filters. (a) Product of two path graphs is a 2D grid. (b) Tensor product of two impulses is a 2D impulse (left). Filtering by the joint adjacency matrix propagates the impulse to neighboring vertices in each path (right). 2D graph spectral filtering.  The input signal is (d,top) the tensor product of an impulse with a smooth function (c) or (d,bottom) a T-V signal: a dynamic mesh ().(e) A separable diffusion filter is the product of domain-specific heat kernels. Separable filters can filter along both axes in unison~(left), or each axis independently (middle / right). (f) Non-separable filter. }
    \label{fig:product_graphs}
 \end{figure*}


%\paragraph{Build a graph on each mode of a tensor, introducing tensor notation as we go}
%\paragraph{Discuss regularization of each graph separately}
%\paragraph{Show that these can be combined into a single Laplacian, i.e. a single graph}
%\paragraph{Early developments: time-vertex, for which there has been a cluster of development}

==> tensors.tex <==
\subsection{Tensors and Tensor Operations}
\label{sec:background/tensors}

%\TODO{introduce tensor notations - calligraphic for tensor, bold uppercase for matrix, bold lowercase for vector?}

%Multiway arrays, also referred to as tensors, are higher-order generalizations of vectors and matrices. 
%A multi-way array or tensor $\T{A} \in \Real^{n_1 \times n_2 \times \cdots \times n_D}$ is of order $D$, or is said to have $D$ \emph{ways} or \emph{modes}. 
%A vector is an order-1 tensor and a matrix is an order-2 tensor.

%From a mathematical perspective, extending from a single sign   al on a graph to multi-way data in the discrete setting, is generalizing from vectors to multi-way tensors. From a GSP perspective the topology underlying each mode of the tensor is a graph.
%As a simple example, in the case of time-varying signals on a sensor network, one mode of the tensor is the network (sensors) and the other mode of the tensor is time.

We adopt the terminology and notation used by \cite{KoldaBader2009}. We call the number of ways or modes of a tensor its {\em order}. Vectors are tensors of order one and denoted by boldface lowercase letters, e.g.\@ $\V{a}$. Matrices are tensors of order two and denoted by boldface capital letters, e.g.\@ $\M{A}$. Tensors of higher-order, namely order three and greater, we denote by boldface Euler script letters, e.g.\@ $\T{A}$. 
If $\T{A}$ represents a $D$-way data array of size $n_1 \times n_2 \times \cdots \times n_D$, we say $\T{A}$ is a tensor of order $D$. We denote scalars by lowercase letters, e.g.\@ $a$. We denote the $i$th element of a vector $\V{a}$ by $\VE{a}{i}$, the $ij$th element of a matrix $\M{A}$ by $\ME{a}{ij}$, the $ijk$th element of a third-order tensor $\T{a}$ by $\ME{a}{ijk}$, and so on. In the special case of an order-3 tensor, $\T{A} \in \Real^{n_1 \times n_2 \times n_3}$, 
%The element $\T{A}_{ijk}$ is the entry in the $i$-th row, $j$-th column and $k$-th fiber.
when an index is fixed in one mode while the indices vary in the other two, this partition is called a \emph{slice}, and it is a matrix. 
\vspace{-0.2cm}
%\minrowclearance 3ex

%Distances can be taken between pairs of slices using different matrix norms on the difference of slices. 

\begin{mdframe}
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth]{figures/tensor.pdf}
    \caption{From left to right: Tensor of order 3 - $\mathcal{T}$, fibers along third mode -  $\mathcal{T}_{ij\cdot}$, slices of first mode -  $\mathcal{T}_{i\cdot\cdot}$, slices of second mode - $\mathcal{T}_{\cdot j \cdot}$. }
    \label{fig:tensor}
    \vspace{-0.2cm}
\end{figure}
\end{mdframe}


It is often useful to reshape a $D$-way array into a matrix or a vector, operations called {\em matricization} and {\em vectorization}, respectively. %There are many ways to reorder a tensor into a matrix or vector. 
In this paper, we use a canonical mode-$d$ matricization, where the mode-$d$ fibers of a $D$-way tensor $\T{A} \in \Real^{n_1 \times n_2 \times \cdots \times n_D}$ become the columns of a matrix $\M{A}_{(d)} \in \Real^{n_d \times n_{-d}}$, where $n_{-d} = \prod_{j \neq d} n_j$. %Recall that the column-major vectorization of a matrix maps a matrix $\M{A} \in \Real^{p \times q}$ to the vector $\V{a} \in \Real^{pq}$ by stacking the columns of $\M{A}$ on top of each other. %, namely $\V{a} = \begin{pmatrix} \M{A}_{:1}\Tra & \M{A}_{:2}\Tra & \cdots & \M{A}_{:q}\Tra \end{pmatrix}\Tra \in \Real^{pq}$. 
In this paper, we take the vectorization of a $D$-way tensor $\T{A}$, denoted $\vec(\T{A})$, to be the column-major vectorization of the mode-1 matriciziation of $\T{A}$. %, namely $\vec(\T{A}) = \vec(\Mz{A}{1}) \in \Real^{n}$, where $n = \prod_{d} n_d$ the total number of elements in $\T{A}$. 
As a shorthand, when there is no ambiguity, we denote the vectorization of a tensor $\T{A}$ by its boldface lowercase version $\V{a}$.

%The Frobenius norm of a $D$-way tensor $\T{A} \in \Real^{n_1 \times n_2 \times \cdots \times n_D}$ is the natural generalization of the Frobenius norm of a matrix, namely it is the square root of the sum of the squares of all its elements,
%\begin{eqnarray*}
%\lVert \T{A} \rVert_{\text{F}} & = & \sqrt{\sum_{i_1 = 1}^{n_1} \sum_{i_2=1}^{n_2}\cdots\sum_{i_D=1}^{n_D} \ME{A}{i_1i_2\cdots i_D}^2}.
%\end{eqnarray*}
%The Frobenius norm of a tensor is equivalent to the $\ell_2$-norm of the vectorization of the tensor, namely $\lVert \T{A} \rVert_{\text{F}} = \lVert \V{a} \rVert_2$.

%\begin{figure*}[th!]
%    \centering
%    \includegraphics[width=\linewidth]{figures/framework_revision1.png}
%    \caption{\TODO{Multiway signal processing frameworks, export as pdf }}
%    \label{fig:framework}
%\end{figure*}
Let $\T{A}$ be a tensor in $\Real^{n_1 \times n_2 \times \cdots \times n_D}$ and $\M{B}$ be a matrix in $\Real^{m \times n_d}$. The {\em d-mode (matrix) product} of the tensor $\T{A}$ with the  matrix $\M{B}$, is the tensor denoted by $\T{A} \times_{d} \M{B} \in \mathbb{R}^{n_1 \times \cdots \times n_{d-1} \times m \times n_{d+1} \times \cdots \times n_D}$ whose $(i_1, i_2, \cdots, i_{d-1}, j, i_{d+1}, \cdots, i_D)$th element is given by 
\begin{eqnarray}
(\T{A} \times_d \M{B})_{i_1\ldots i_{d-1} j i_{d+1} \cdots i_D} & = & \sum_{i_d = 1}^{n_d} \ME{a}{i_1i_2\cdots i_D}\ME{b}{j i_d}, \quad \textrm{for } j \in \{1, \ldots, m\}
\end{eqnarray}
The vectorization of the $d$-mode product $\T{A} \times_{d} \M{B}$ can be expressed as
%\begin{equation}
%\begin{split}
%\label{eq:vec_identity}
%\vec (\T{A} &\times_d \M{B}) 
% =   \\ &(\M{I}_{n_D} \Kron \cdots \Kron \M{I}_{n_{d+1}}\Kron \M{B} \Kron \M{I}_{n_{d-1}} \Kron \cdots \Kron \M{I}_{n_1} )\V{a},
%\end{split}
%\end{equation}
\begin{equation}
\begin{split}
\label{eq:vec_identity}
\vec (\T{A} &\times_d \M{B}) 
 =  (\M{I}_{n_D} \Kron \cdots \Kron \M{I}_{n_{d+1}}\Kron \M{B} \Kron \M{I}_{n_{d-1}} \Kron \cdots \Kron \M{I}_{n_1} )\V{a},
\end{split}
\end{equation}
where $\M{I}_p$ is the $p$-by-$p$ identity matrix and $\Kron$ denotes the Kronecker product between two matrices. %The identity given in \Eqn{vec_identity} generalizes the well known formula for the column-major vectorization of a product of two matrices, namely $\vec(\M{B}\M{A}) = (\M{I}\Kron\M{B})\V{a}$.



%\subsection{Tensor Products}
%\label{sec:background/tensorproducts}

We generate multi-way operators by using the tensor product $\Kron{}$ throughout this paper. %, which for finite settings is known as the Kronecker product.
Briefly, the tensor product of two vector spaces $V$ and $W$ is $H= V\Kron{}W$. 
Tensor products enable us to generalize linear operators from the classical setting to multilinear operators in the tensor setting. %In addition, in Sec.~\ref{sec:structures/productgraphs} we show how different graph topologies give rise to different eigensystems calculated using tensor products between the eigenpairs of the single way modes. 
 
% In the following we explain how to calculate the eigensystems of product spaces, such as tensors, using tensor products.
% This will enable us to generalize the GSP operators which rely on the eigendecomposition of the graph Laplacian, to the multi-way setting.
 %$H$ is a space equipped with the bilinear map $\varphi:V\times W \mapsto V\Kron W$. This enables one to treat multilinear operators $S:V\times W\mapsto Z$ for some vector space $Z$ as a linear map $S^\prime:H\mapsto Z$ such that $S = S^\prime\circ \varphi$.
We focus on the tensor product of general Hilbert spaces $\mathcal{H}^{(k)}, k=1,\ldots, d$, i.e. complete spaces equipped with an inner product. The tensor product of Hilbert spaces generates unique linear operators on the product space $\mathcal{H} = \Kron_{k=1}^d \mathcal{H}^{(k)}$. This structure admits a multilinear operator over the Cartesian product: $S:\mathcal{H}^{(1)} \times \cdots \times \mathcal{H}^{(d)}\mapsto Z$, which is useful for considering multi-way structures in total or as a set of independent vector spaces parameterized by the others. In graph signal processing we are typically interested in finite vector spaces such as $\mathcal{H}^{(k)} = \Complex^{n_k}$. If each $\mathcal{H}^{(k)}$ is finite, their tensor product $\mathcal{H} = \Kron_{k=1}^d \mathcal{H}^{(k)}$ is of dimension $\prod_{k=1}^d \mathrm{dim}(\mathcal{H}^{(k)}).$ 

One example of the finite tensor product is the Kronecker product, which produces the matrix of a tensor product with respect to a standard basis. 
%\begin{align*} 
%\langle (v_1, v_2),(u_1, u_2)\rangle = \langle v_1,u_1\rangle_1 \, \langle v_2,u_2\rangle_2 \quad \\ \mbox{for all } v_1,u_1 \in \mathcal{H}^{(1)} \mbox{ and } v_2,u_2 \in \mathcal{H}^{(2)}, 
%\end{align*} 
%, i.e. if $S:\mathcal{H}^{(1)} \times \ldots \times \mathcal{H}^{(d)}\mapsto Z$, then we can examine the structure of one axis by ``fixing'' an axis (or mode) of $S$.  For example,  $$S(\cdot,x^{(2)},\ldots,x^{(k)})=S^{(1)}(\cdot)S^{(2)}(x^{(2)})\ldots S^{(d)}(x^{(d)})$$ (by bilinearity) is itself a linear map on the first Hilbert space, i.e. $S^{(1)}:\mathcal{H}^{(1)}\mapsto Z$. 
%It is a generalization of the outer product of vectors $\V{x}\V{y}^*$ for $\V{x}\in\Complex^{m}$ and $\V{y} \in \Complex^{n}$. 
%The Kronecker product of two matrices $\M{A}^{(1)} \in \Complex^{n_1\times m_1}$ and $\M{A}^{(2)} \in \Complex{}^{n_2\times m_2}$ is the $n_1n_2\times m_1m_2$ matrix 
%$${\displaystyle \Mn{A}{1}\otimes \Mn{A}{2}  ={\begin{bmatrix}\MnE{A}{1}{11}\Mn{A}{2} &\cdots &\MnE{A}{1}{1m_1}\Mn{A}{2}\\\vdots &\ddots &\vdots \\\MnE{A}{1}{n_11}\Mn{A}{2} & \cdots&\MnE{A}{1}{n_1m_1}\Mn{A}{2} \end{bmatrix}}.}$$
The Kronecker product is associative, so the Kronecker product of the sequence of $d$ matrices $\M{A}^{(k)} \in \Complex^{n_k}$ for $k=1,\ldots,d$, is 
%\begin{equation}
%\begin{split}
%\M{A}^{\otimes} = \bigotimes_{k=1}^d \M{A}^{(k)} &=  \M{A}^{(1)}\bigotimes_{k=2}^d \M{A}^{(k)} = \left(\bigotimes_{k=1}^{d-1} \M{A}^{(k)}\right)\Kron \M{A}^{(d)}\\ &= \M{A}^{(1)}\Kron \ldots \Kron \M{A}^{(d)}.
%\label{eq:general_kronecker_product}
%\end{split}
%\end{equation}
\begin{equation}
\begin{split}
\M{A}^{\otimes} = \bigotimes_{k=1}^d \M{A}^{(k)} =  \M{A}^{(1)}\bigotimes_{k=2}^d \M{A}^{(k)} = \left(\bigotimes_{k=1}^{d-1} \M{A}^{(k)}\right)\Kron \M{A}^{(d)} = \M{A}^{(1)}\Kron \cdots \Kron \M{A}^{(d)}.
\label{eq:general_kronecker_product}
\end{split}
\end{equation}

%A related notion to the Kronecker product is the Kronecker sum.  We will use this to generate combinatorial graphs from tensor modes. The Kronecker sum of $\M{A}^{(1)}$ and $\M{A}^{(2)}$ is the $n_1n_2\times n_1n_2$ matrix $\M{A}^{(1)}\oplus\M{A}^{(2)} =  \M{A}^{(1)}\Kron{}\M{I}_{n_2}  \M{I}
%_{n_2} \Kron{}\M{A}^{(2)}.$ Defining $\M{A}^{(1)}\oplus\M{A}^{(2)}$ in this order ensures that it commutes with $\M{A}^{(1)}\Kron\M{A}^{(2)}$ without permutation.  
% A general Kronecker sum of $d$ matrices $\M{A}^{(k)} \in \Complex^{n_k}$ for $k=1,\ldots,d$ is 
% \begin{align}
% \M{A}^{\oplus}= \bigoplus_{k=1}^d \M{A}^{(k)} = \sum_{k=1}^{d} \M{I}_{n_{>k}}\Kron{}\M{A}^{(k)}\Kron{}\M{I}_{n_{<k}},\label{eq:general_kronecker_sum} \text{where} ~ n_{>k} = \prod_{\ell=k+1}^d n_\ell, ~ \text{and}~ n_{<k} = \prod_{\ell=1}^{k-1} n_\ell\nonumber.
% \end{align}
%  \begin{align}
% \M{A}^{\oplus}= \bigoplus_{k=1}^d \M{A}^{(k)} = \sum_{k=1}^{d} \M{I}_{n_{>k}}\Kron{}\M{A}^{(k)}\Kron{}\M{I}_{n_{<k}},\label{eq:general_kronecker_sum} \\ \text{where} ~ n_{>k} = \prod_{\ell=k+1}^d n_\ell, ~ \text{and}~ n_{<k} = \prod_{\ell=1}^{k-1} n_\ell\nonumber.
% \end{align}

For more details on tensors and general applications of tensor analysis we refer the interested reader to the related reviews on multi-way data analysis with multilinear methods, tensor decompositions and their applications to signal processing in a non-GSP setting~\cite{acar2009unsupervised,KoldaBader2009,Cichocki2015}.
%In Section~\ref{} we review latent factor discovery in tensor data using both linear and nonlinear techniques (which is not covered in~\cite{acar2009unsupervised}).

%\TODO{figure for tensor product graph}

